Did I delete my cookies? Cookies respawning with browser fingerprinting

Stateful and stateless web tracking gathered much attention in the last decade, however they were always measured separately. To the best of our knowledge, our study is the first to detect and measure cookie respawning with browser and machine fingerprinting. We develop a detection methodology that allows us to detect cookies dependency on browser and machine features. Our results show that 1,150 out of the top 30, 000 Alexa websites deploy this tracking mechanism. We further uncover how domains collaborate to respawn cookies through fingerprinting. We find out that this technique can be used to track users across websites even when third-party cookies are deprecated. Together with a legal scholar, we conclude that cookie respawning with browser fingerprinting lacks legal interpretation under the GDPR and the ePrivacy directive, but its use in practice may breach them, thus subjecting it to fines up to 20 million euro.

==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> limitation.tex <==
\NB{better use "key" instead of "name" as it's a more standard terminology. You need to add a limitation explaining how cookies are set and such ownership assumption has limitations.}

==> rebuttal.tex <==
\textbf{\#134A:}\\
\textbf{Cross-site tracking:}
Through the paper, we study both respawning of first and third- party cookies that can be used for cross-site tracking.
We found that 875 (46.47%) of the respawned cookies are used for cross-site tracking (Section 5.5).

\textbf{Selection of fingerprinting attributes:}
Our goal is not to be exhaustive on the studied fingerprinting features as the number of features used for fingerprinting is continuously increasing.
Instead, we limited our study to 8 features that are commonly used and that we can easily spoof. 

\textbf{Low-entropy fingerprinting attributes:}
Our methodology allows us to detect dependency between the fingerprinting feature and the respawned cookie.
However, given that we analyze a limited number of fingerprinting features, 
What we detect as features used for respawning cookies could be used in combination with other features out of the scope of the paper.

\textbf{Usage of cookies and fingerprint:}
Fingerprinting tracking techniques are not  stable over time.
%expensive performance side
Cookies are simpler to manage, they are sent automatically by the browser with every request, and persistent as long as they are not erased nor expired.
Using the combination of both fingerprinting and cookies, companies can assess the fingerprint variation, and ensure a long term tracking even after the cleaning browser storage (By default in Firefox, INSERT cleaning the browser includes cleaning all browser storage).
Furthermore, using fingerprint and first party cookies can insure a persistent and stable cross-site tracking as explained in Section 5.5.2.



==> trash.tex <==
\section{Trash}
\subsection{Methodology trash}

\begin{figure}[!thp]
\centering
\subfloat[%Comparing to 
{Websites prevalence}\label{fig:compareELEP}]{\includegraphics[width=0.5\textwidth]{figures/website_prevalence.PNG}}

\subfloat[%Comparing to 
Cookies prevalence\label{fig:compareDISC}]{\includegraphics[width=0.5\textwidth]{figures/cookie_prevalence.PNG}}
\caption{ {\normalfont}
{Prevalence of \ourmethod}. \textit{We detected  {\respcookies} respawned cookies that belong to {\respwebsites}  websites.}  } %({\totaldomainssucc} domains).}
\label{fig:overviewT} 
\end{figure} 


\begin{table}[!htbp]
    \centering
    \hspace{ -.3 cm}
    \begin{tabular}{|p {1.9cm}|p {5.2 cm}|}
    \hline
    \textbf{Categories} & \textbf{Host $\rightarrow$ Website} \\ \hline
Internet Services $\rightarrow$  Pornography
&   \makecell{ trafficjunky.net $\rightarrow$ keezmovies.com \\ trafficjunky.net $\rightarrow$ e-hentai.org }  \\ \hline
 Parked Domain $\rightarrow$  Pornography  &  servingmillions.com $\rightarrow$ sex.com   \\ \hline
  Content Server $\rightarrow$  Pornography  &  realsrv.com $\rightarrow$ bravotube.net   \\ \hline
 Pornography $\rightarrow$  Pornography  &  a.adtng.com $\rightarrow$ sxyprn.com   \\ \hline
\hline
\hline
 Business  $\rightarrow$   Health  &  rubiconproject.com  $\rightarrow$  self.com  \\ \hline
 Internet Services  $\rightarrow$   Health  & 
 \makecell{casalemedia.com  $\rightarrow$  andhrajyothy.com  \\ casalemedia.com  $\rightarrow$  self.com  } \\
\hline
\hline

    \end{tabular}
    \caption{Third party cookies respawned in sensitive websites.}
    \label{tab:sensitive}
\end{table}


\subsection{Results trash}


\iffalse
\begin{table}[!htbp]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Host} & \textbf{Key} & \textbf{Occurence} \\ \hline
    \hline
rubiconproject.com  &  rsid  &  515 \\ 
casalemedia.com  &  CMPS  &  288 \\ 
smartadserver.com  &  pbw  &  111 \\ 
rubiconproject.com  &  vis15  &  68 \\ 
pubmatic.com  &  pi  &  62 \\ 
casalemedia.com  &  CMDD  &  70 \\ 
quantserve.com  &  d  &  53 \\ 
addthis.com  &  loc  &  69 \\ 
rubiconproject.com  &  vis2  &  58 \\ 
casalemedia.com  &  CMPRO  &  30 \\ \hline
    \end{tabular}
    \caption{Top 10 third party respawned cookies}
    \label{tab:basicT}
\end{table}
\fi
%\IF{Presence of the cookies in the visited sites (\% of profile) exp of websites where it happens}



\begin{table*}[!htbp]
    \centering
    \begin{tabular}{|c|c|c|c|c|p {2.5 cm}|}
    \hline
    \textbf{Host} & \textbf{Key} & \textbf{Purpose} &  \textbf{Occurence} & \textbf{Country} & \textbf{Organisation} \\ \hline
casalemedia.com  &  CMPS & Targeting/Advertising  &  288  &  CA  &  Index Exchange Inc.  \\ \hline
smartadserver.com  &  pbw & Targeting/Advertising  &  111  &  fr  &  Smartadserver  \\ \hline
casalemedia.com  &  CMDD & Targeting/Advertising  &  77  &  CA  &  Index Exchange Inc.  \\ \hline
addthis.com  &  loc & Targeting/Advertising  &  69  &  US  &  REDACTED FOR PRIVACY  \\ \hline
casalemedia.com  &  CMPRO & Targeting/Advertising  &  30  &  CA  &  Index Exchange Inc.  \\ \hline
tvn24.pl  &  AWSALBCORS & Strictly Necessary  &  29  &  None  &  None  \\ \hline
ohio.gov  &  AWSALBCORS & Strictly Necessary  &  20  &  None  &  None  \\ \hline
gumgum.com  &  loc & Targeting/Advertising  &  18  &  US  &  GumGum  \\ \hline
eyeota.net  &  SERVERID & Strictly Necessary  &  18  &  SG  &  Eyeota Pte Ltd  \\ \hline
audible.fr  &  s\_sess & Performance  &  6  &  None  &  None  \\ \hline
nuggad.net  &  nid & Targeting/Advertising  &  5  &  None  &  None  \\ \hline
pubmatic.com  &  KTPCACOOKIE & Targeting/Advertising  &  3  &  US  &  PubMatic, Inc.  \\ \hline
smartadserver.com  &  csync & Targeting/Advertising  &  3  &  fr  &  Smartadserver  \\ \hline
a.adtng.com  &  RNLBSERVERID & Strictly Necessary  &  3  &  LU  &  Whois Privacy (enumDNS dba)  \\ \hline
ads2.newmedia.az  &  OAGEO & Targeting/Advertising  &  3  &  None  &  None  \\ \hline
ads2.adviad.com  &  OAGEO & Targeting/Advertising  &  3  &  GE  &  None  \\ \hline
mheducation.com  &  s\_ppv & Performance  &  3  &  US  &  McGraw-Hill Global Education Holdings, LLC  \\ \hline
weborama.fr  &  wbo\_temps\_reel & Targeting/Advertising  &  3  &  None  &  None  \\ \hline
us.ck-ie.com  &  CID & Targeting/Advertising  &  3  &  US  &  SMARTYADS Inc  \\ \hline
michaelkors.fr  &  s\_ppv & Performance  &  2  &  None  &  None  \\ \hline
    \end{tabular}
    \caption{Top 20 cookies (host,key) violating GDPR. \textit{Occurrence: presents the number of websites where the cookie (host,key) is respawned. Purpose: cookiepedia corresponding purpose. Country and organisation: Country and registered organisation extracetd using whois library \cite{}.}}
    \label{tab:viola_exp}
\end{table*}


\iffalse

\IF{To update the table with owners}
\begin{table}[!htbp]
    \centering
    \begin{tabular}{|p{3.5cm}|p{1cm}|p{1.7cm}|}
    \hline
\textbf{(Host, key)} & \textbf{Occu-rrence} & \textbf{Purpose}   \\ \hline
(rubiconproject.com, rsid)  &  515 & Unknown \\ \hline
(assets.rrz.unihamburg-.de, \_fionaapp\_session)  &  33 & Unknown  \\ \hline
(bh.contextweb.com ,  INGRESSCOOKIE) &  24  & Unknown\\ \hline
(bedbathandbeyond.com,  s\_sess)  &  9  & Performance \\ \hline
(key.com, s\_sess)  &  6 & Performance \\ \hline
(audible.fr, s\_sess)  &  6 & Performance \\ \hline
(www.dnb.no,    portal\_scriptable)  &  6 & Unknown  \\ \hline
(enterprise.com,    s\_sess)  &  5 & Performance  \\ \hline
(subway.com,    s\_sess)  &  4  & Performance \\ \hline
(snapdeal.com,    s\_sess)  &  3 & Performance  \\ \hline

    \end{tabular}
    \caption{Top 10 respawned session cookies. \normalfont{ \textit{Occurrence}: presents the number of websites where the cookie (host,key) was respawned. Purpose: cookiepedia corresponding purpose.}}
    \label{tab:session}
\end{table}

Among the top respawned session cookies, 6 have as key s\_sess.
The s\_sess cookie is known as session web analytics cookies, provided and managed by Adobe Inc., and used to collect information about how visitors use websites.
This cookie is owned by adobe, and set by adobe script on different third party context, hence, it is stored with different hosts. 


\fi





\clearpage

\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/metho.png}
    \caption{Methodology used to extract scripts responsible of respawning.}
    \label{fig:method}
\end{figure*}






\subsection{Panorama of respawned cookies}




\begin{table*}[!htp]
    \centering
    \begin{tabular}{|p{3.5 cm}|p{ 3 cm}|p {2cm}| p {1.5cm}|p {4cm}|}
    \hline
    \textbf{Host} & \textbf{Key} & \textbf{Occurrence} & \textbf{Country} & \textbf{Organization}   \\ \hline

rubiconproject.com  &  rsid  &  372  &  US  &  The Rubicon Project, Inc.  \\ \hline
casalemedia.com  &  CMPS  &  109  &  CA  &  Index Exchange Inc.  \\ \hline
smartadserver.com  &  pbw  &  76  &  fr  &  Smartadserver  \\ \hline
casalemedia.com  &  CMDD  &  68  &  CA  &  Index Exchange Inc.  \\ \hline
pubmatic.com  &  pi  &  57  &  US  &  PubMatic, Inc.  \\ \hline
quantserve.com  &  d  &  53  &  US  &  Quantcast  \\ \hline
rubiconproject.com  &  vis15  &  52  &  US  &  The Rubicon Project, Inc.  \\ \hline
rubiconproject.com  &  vis2  &  44  &  US  &  The Rubicon Project, Inc.  \\ \hline
assets.rrz.uni-hamburg.de  &  \_fionaapp\_session  &  33  &  None  &  None  \\ \hline
casalemedia.com  &  CMPRO  &  28  &  CA  &  Index Exchange Inc.  \\ \hline
bh.contextweb.com  &  INGRESSCOOKIE  &  20  &  US  &  PulsePoint  \\ \hline
eyeota.net  &  SERVERID  &  16  &  SG  &  Eyeota Pte Ltd  \\ \hline
addthis.com  &  loc  &  15  &  US  &  REDACTED FOR PRIVACY  \\ \hline
smartadserver.com  &  sasd  &  14  &  fr  &  Smartadserver  \\ \hline
realsrv.com  &  tag-banner  &  12  &  US  &  See PrivacyGuardian.org  \\ \hline
aralego.com  &  sspid  &  10  &  TW  &  None  \\ \hline
ohio.gov  &  AWSALB  &  10  &  None  &  None  \\ \hline
ohio.gov  &  AWSALBCORS  &  10  &  None  &  None  \\ \hline
bedbathandbeyond.com  &  s\_sess  &  9  &  US  &  Bed Bath \& Beyond Procurement Co. Inc.  \\ \hline
justpremium.com  &  jpxumatched  &  8  &  NL  &  REDACTED FOR PRIVACY  \\ \hline
    \end{tabular}
    \caption{Top 20 respawned  cookies.  \textit{Occurrence: presents the number of websites where the cookie (host,key) is respawned. In total we detect 1,748 websites where at least one cookie was respawned. }}
    \label{tab:respawned}
\end{table*}



Table \ref{tab:respawned} presents the top 20 respawned cookies. 
For each cookie,  we extract its occurrence, organization  and country of registration 
using the whois library~\cite{whois}.

We found that using the \textit{rsid} cookie alone, \textit{rubiconproject.com} persistently track the user on $372$ (2.66\%) websites.
This percentage becomes more important if we consider the company instead of the domain.
By considering companies instead of domains, we found that the owner of rubiconproject.com, \textit{The Rubicon Project} respawn cookies via browser fingerprinting in 485  (3.46\%) websites.





\iffalse
%\subsection{Respawned cookies characteristics}
The 29WP \cite{X} states that  session cookies are  needed to provide a service explicitly
requested by the user, for the duration of a session.
They are used to keep track of the user’s input (session-id) when
filling online forms over several pages, or as a
shopping cart, to keep track of the items the user has selected by clicking on a button.
Such cookies can  be  exempted  from  informed  consent.

Using {\ourmethod} one can recreate session cookies after the expiration of the user session.
Hence, such cookies can be used for a longer duration in a persistent way. 
We found that out of $1,058$ respawned cookies, 290 (27.41\%) are session cookies.
The 290 respawned cookies instances (host,key,value) belongs to 206 cookies (host,key).

\begin{table}[!htbp]
    \centering
    \begin{tabular}{|p{3cm}|p{2cm}|p{2cm}|}
    \hline
\textbf{Host} & \textbf{Key} & \textbf{Occurrence}   \\ \hline
rubiconproject.com  &  rsid  &  372  \\ \hline
assets.rrz.uni-hamburg.de  &  \_fionaapp\_session  &  33  \\ \hline
bh.contextweb.com  &  INGRESSCOOKIE  &  20  \\ \hline
bedbathandbeyond.com  &  s\_sess  &  9  \\ \hline
key.com  &  s\_sess  &  6  \\ \hline
audible.fr  &  s\_sess  &  6  \\ \hline
enterprise.com  &  s\_sess  &  5  \\ \hline
discovery.co.za  &  dtLatC  &  3  \\ \hline
ads2.adviad.com  &  OAGEO  &  3  \\ \hline
www.ionos.com  &  WEB\_FONTS  &  3  \\ \hline

    \end{tabular}
    \caption{Top 10 respawned session cookies.  \textit{Occurrence}: presents the number of websites where the cookie (host,key) was respawned.}
    \label{tab:session}
\end{table}


%A session cookie get deleted when the user close her browser.
%Unlike session cookies where no expiration date is associated to the cookie, 
%persistent cookies have an expiration date and are get deleted within this last.
Table \ref{tab:session} presents the top 10  respawned session cookies.
Rubiconproject.com rsid cookies has been respawned in 372 websites.
Rubiconproject states that: 

\say{\textit{rsid}: Session cookie that contains information about a device, including region (derived from IP address, not geolocation data), operating System, browser, etc., that is used during the ad inventory sale process} \cite{rubicon}.
\fi
\iffalse
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/host_catego.png}
    \caption{Top 20 respawned cookies hosts categories. \textit{ The respawned cookies are set by 496 unique hosts.}}
    \label{fig:hostCat}
\end{figure}
\fi

\subsection{Value length analysis}
A cookie value is composed of US-ASCII characters excluding control characters, Whitespace, double quotes, comma, semicolon, and backslash \cite{encoding}. 
Many companies perform URL encoding on cookie values even though it's not required by the RFC specification.
Therefore,  we  URL decode cookies values before comparing their length. 

Figure \ref{fig:length} presents the comparison of values length between  the $1,058$ respawned cookies and the remaining $299,816$ non spoofed cookies. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/length.png}
    \caption{Comparison of values length of respawned and non respawned cookies. \textit{Respawn cookies: cookies detected by {\ourmethod}. In total we detected $1,058$ respawn cookie. }}
    \label{fig:length}
\end{figure}

We notice that non respawn cookies tend to have a higher value length.
The median and the upper quartil that respectively mark 50\% and 75\% of the data are higher for non respawn cookies.

We also noticed that cookies with values of length 1 are respawned as well.
We found that $65$ cookies out of $1,058$ have values of length 1 ($6.14\%$).
We grouped respawned cookies of length 1 by keys,
and we analyzed the top 3 recurrent cookies keys (Table \ref{tab:keys}).


\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{5 cm}|p{2cm}|}
    \hline
         \textbf{Keys} & \textbf{Occurrence} \\ \hline
         \_ym\_visorc\_* & 19  \\ \hline
         dtLatC  &  14  \\ \hline 
         pushNotification-shownCount-* & 8 \\
         \hline
    \end{tabular}
    \caption{Top 3  keys used with respawned cookies of length 1.
    \textit{These 3 keys are used with 63.07\% of respawned cookies with length 1. Occurrence: the number of cookies using the key. *: A numeric value.    }}
    \label{tab:keys}
\end{table}

\paragraph{\_ym\_visorc\_*:}
according to the cookie policy \url{https://www.vostockcapital.com/en/cookies-policy-for-website/},
\_ym\_visorc\_* is used with yandex.ru and contains a unique identifier that is assigned to each browser to track user interaction with the website.
This identifier is stored as part of the cookie key that we mark as *.

\textit{Is \_ym\_visorc\_* cookie always respawned? }
In our dataset, \_ym\_visorc\_* have 612 (host,key,value) instance in our \CMinit.
However it only has 2 different cookie values \{w and b\}.
Out of 612 cookies instances only 19(3.10\%) were detected as respawned.

\textit{Is \_ym\_visorc\_* always respawned with the same feature?}
No, \_ym\_visorc\_* cookies are respawned with different features.

\textbf{Conclusion:} \_ym\_visorc\_* cookie contains an identifier as part of the cookie key.
This identifier is respawned after cleaning the browser, in fact, we re-detect the same host, key in the different crawls.
However, our identification of feature related cookies does not apply to this specific case since it's built based on identifiers stored in the cookie value not in it's key.


\paragraph{dtLatC: }
No  info about the usage of the cookie found in the cookie policies.

\textit{Is dtLatC cookie always respawned? }
In our dataset, dtLatC key appears in  170 (host,key,value) instance in our \CMinit.
Out of 170 cookies instances only 15 (among which 14 use a value of length 1) were detected as respawned.
DtLatC has 82 different numeric values in the \CMinit.


\paragraph{pushNotification-shownCount-*}
No  info about the usage of the cookie found in the cookie policies.

\textit{Is pushNotification-shownCount-* cookie always respawned? }
In our dataset, pushNotification-shownCount-* key appears in  113 (host,key,value) instance in our \CMinit.
Out of 113 cookies instances only 8 were detected as respawned.
pushNotification-shownCount-* has 2 different numeric values in the \CMinit \{0,1\}.



\begin{figure*}[!htb]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/length_perfeature.png}
    \caption{Comparison of values length of respawned and non respawned cookies. \textit{DNT respawn cookies: cookies respawned using the Do not track feature.  Lang respawn cookies: cookies respawned using the accept language feature. IP respawn cookies: cookies respawned using the IP address feature. TZ respawn cookies: cookies respawned using the time zone feature. UA respawn cookies: cookies respawned using the user agent feature. GEO respawn cookies: cookies respawned using the geolocation feature.}}
    \label{fig:length}
\end{figure*}












\subsection{Respawn cookie value analysis}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|p{5.5 cm}|p{2 cm}|}
    \hline
    \textbf{Values} & \textbf{Occurrence} \\ \hline
  eJw9jU1O \dots ww+bA==  &  15 \\ \hline 

\dots Gecko/20100101 Firefox/68.0  &  7 \\ \hline 

3  &  5 \\ \hline 

66c0f892e4c0f7a6757a87e9144ac554  &  5 \\ \hline 

050118664680201001016800768136624  &  5 \\ \hline 

1  &  4 \\ \hline 

pA8AAGsis1cJsL5XAYh6wwA=  &  4 \\ \hline 

w  &  4 \\ \hline 

4422882a37b52eda8d4295d5b6df464b  &  3 \\ \hline 

b  &  3 \\ \hline 

{"minAnalytics":"{\"clicks\":[]}"}  &  3 \\ \hline 

fmt5fa9n124oyj9ztereesa  &  3 \\ \hline 

435846058  &  3 \\ \hline 

Firefox-68  &  3 \\ \hline 

62213378222363201731411483358512  &  3 \\ \hline 

{"minAnalytics":"{\"clicks\":[]}","\_minEE1":"[]"}  &  3 \\ \hline 

zZtcdzmV1DO+eY8HT3P0lv0CLB \dots  &  2 \\ \hline 

2112:15970007659641800  &  2 \\ \hline 

2107:15976126602880602  &  2 \\ \hline 

uZr6boikZRuObrfiPkDlZ \dots  &  2 \\ \hline 

    \end{tabular}
    \caption{Top 20 values used with cookies respawned using the user agent. \textit{Occurrence: number of times the cookie value was used with the 1,058 respawned cookies.}}
    \label{tab:topua}
\end{table}




\paragraph{Cookies respawned using all features combined}

We found that 8 cookies were respawned using all features combined.
\begin{table}[!htp]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
\textbf{Host} & \textbf{Key} & \textbf{Value} \\ \hline
  .citationmachine.net &  al\_ff &  eyJhbGxvY2F0aW9 \dots \\ \hline
 .citationmachine.net & ad\_config\_version &  8-6-one-trust-new-iab-62-control\\ \hline
openclassrooms.com &  AWSELB &  85E3E1750E02C5A \dots \\ \hline
openclassrooms.com &  AWSELBCORS & 85E3E1750E02C5A\dots \\ \hline
.casalemedia.com & CMPRO & 1857 \\ \hline
bh.contextweb.com &  INGRESSCOOKIE &  7390e0f465cddccf \\ \hline
.quantserve.com &  d &  EC0BGgGMIYqsMM2MgQrLjRA \\ \hline
.casalemedia.com &  CMPRO &  234 \\ \hline

    \end{tabular}
    \caption{Respawned cookies using all features combined}
    \label{tab:my_label}
\end{table}






\iffalse
%The detection of features related cookies is done in 5 sequential rounds.

\begin{figure*}[th!]
\centering
\subfloat[%Comparing to 
{Websites prevalence}\label{fig:compareELEP}]{\includegraphics[width=0.5\textwidth]{figures/stable_sites_cumu.png}}
\subfloat[%Comparing to 
Cookies prevalence\label{fig:compareDISC}]{\includegraphics[width=0.5\textwidth]{figures/stable_cumu.png}}
\caption{ {\normalfont}
%A: requests blocked by the filtering list and not detected by our method, B: requests blocked the filtering list and detected by our method, C; requests detected only by our method. \emph{The analysis is done on the {\totaldomainssucc} successfully crawled domains with a total of $4,216,454$ third party requests.
%Efficiency 
Stability of {\ourmethod} through the 5 rounds } %({\totaldomainssucc} domains).}
%
%\subfloat[Comparing to EasyList and EasyPrivacy]{\includegraphics[width=0.4\textwidth]{Figures/detection_blocking.png}} 
%\subfloat[Comparing to Disconnect]{\includegraphics[width=0.4\textwidth]{Figures/diconnect.png}}
%\caption{ {\normalfont} A: requests blocked by the filtering list and not detected by our method, B: requests blocked the filtering list and detected by our method, C; requests detected only by our method. \emph{The analysis is done on the first 8,425 successfully crawled domains with a total of $4,275,704$ third party requests.}} 
%
\label{fig:stable} 
\end{figure*} 

Figure \ref{fig:stable} presents the cumulative distribution function of the intersection of respawned cookies and websites at each round.
In round 2, we can see that we have a drop of number of common respawned cookies.
However, this drop became less important at each round,
until it becomes stable between round 4 and round 5.
Cookies appearing in the 5 rounds, are the cookies that we refer to as \textit{strongly dependent on the feature}. These cookies are respawned and depend on the feature in all 5 rounds.







\fi




\subsection{Evaluation criteria}
\label{sec:criteria}
The 29WP (WP194)~\cite{} exposes that "it is the purpose (and its practical implementation) that must be used to determine whether or not a cookie can be exempted from consent". While analysing the cookies present on a website, any auditor needs to capture the \emph{purpose} of each cookie. The defined purpose can then help to determine whether processing is legally compliant, what safeguards the GDPR imposes, and which legal basis can be used.

%\AL{you don't use the same order here and in the paragraph below. Also, the provenance of cookies is not the purposes of cookies. You must be consistent in your terms. Also if WP194 refer to provenance, with cookiepdia you are not looking at that, so it is misleading.}

%\AL{once you fix a point, just comment both the question and your answer. It must not appear in the pdf anymore, but should be searchable in the .tex as a comment.}



\begin{table*}[!h]
  \centering
  \begin{tabular}{ | p{.65cm} | c  | c | p {.5cm} |}
    \hline
    &  Session & Persistent  & \\ \hline
        \begin{turn}{90}First-Party\end{turn}
 
    & 
    \begin{minipage}{.4\textwidth}
      \includegraphics[width=\linewidth]{figures/purpose_fp_short.png}
      \caption*{ 368 (19.54\%) cookies}
    \end{minipage}
    &
    \begin{minipage}{.4\textwidth}
      \includegraphics[width=\linewidth  ]{figures/purpose_fp_persistent.png}
      \caption*{640 (33.90\%) cookies}
    \end{minipage}
    & 
    \begin{turn}{90}1008 (53.53\%)\end{turn}

    

    \\ \hline
    
    \begin{turn}{90}Third-Party\end{turn}
    & 
    \begin{minipage}{.4\textwidth}
      \includegraphics[width=\linewidth]{figures/purpose_tp_short.png}
      \caption*{97 (5.15\%) cookies}
    \end{minipage}
    
    &
    \begin{minipage}{.4\textwidth}
      \includegraphics[width=\linewidth]{figures/purpose_tp_persistent.png}
      \caption*{778 (41.32\%) cookies}
    \end{minipage}
    & 
     \begin{turn}{90}875 (46.47\%)\end{turn}

    \\ \hline
    Total & 465 (24.69\%) &  1,418 (75.31\%) &  
            \begin{turn}{45}1883\end{turn}
  
    \\ \hline
  \end{tabular}
  \caption{Overview of respawned cookies characteristics}\label{tab:overview_resp}
\end{table*}


The 29WP WP194 adds two characteristics~\cite{} that can contribute to whether cookies are exempted and non-exempted of consent: (1) Duration of cookies and (2) Provenance of cookies. Hereby we analyse how the purpose and these  additional criteria (duration and provenance) are applied to respawned cookies and then we provide the foregoing results (Table \ref{tab:overview_resp}).


\subsubsection{Cookiepedia purposes and respawned cookies}

%\noindent
%\textbf{Cookiepedia pre-categorized purposes.}

\CS{I have a table to insert here with Cookiepedia purposes and the need for consent}

\noindent
\textbf{Cookiepedia purposes and respawned cookies.}
We analysed the purposes of respawned cookies to understand whether they are subject to consent or not. 
%\NB{subject TO consent}
%As the 29WP (WP194) exposes, ‘it is the purpose and the specific implementation or processing being achieved that must be used to determine whether or not a cookie can be exempted from consent’ \cite{EDPB-4-12}.
To extract the purpose of the {\respcookies} respawned cookies, we  automatized the cookiepedia service \cite{cookiepedia}.
We made an automatic search of the cookie purpose based on cookie keys.
Cookie keys alone do not guarantee the uniqueness of the cookie because a key can be shared by several cookies.
%\AL{you are still using the terms name and key inconstantly. This problem must have been solved and fixed in the entire document. I recommend to use the term key everywhere (but if name is more standard, use it).}
%\IF{Sorry, I am fixing it in the full paper. I will keep key.}
 However, some of the most common cookies are set by popular platforms, and for  these cookies, the key alone can  identify  the purpose of the cookie with a high certainty.
%\AL{what do you mean by name, do you mean key?}

%\NB{I am not sure it's clear to the reader what is "cookies keys".}
We define a cookie with the triplet (host, key, value).
\AL{you should probably start with this sentence. The logic is: 1) what is a unique cookie 2) why we want to consider the key alone to classify a cookie purpose 3) can we use the key alone (here you give the numbers)}
The {\respcookies} respawned cookies use a set of $621$ unique keys. 
Out of the $621$ unique keys, $506$ (81.48\%) were used with a single host. Hence, the cookie key alone is a distinguishing factor in our respawned cookies dataset.

For every key, we sent an automatic request to cookiepedia, then we extracted the corresponding purpose.
Out of  $621$ unique keys, $432$ were  classified by cookiepedia. These $432$ keys correspond to $1,665$ respawned cookies.
\NB{How many of the 432 keys have different hosts?}

Respawned cookies are grouped into 6 different categories:
\begin{itemize}
    \item Not found: The search of the cookie purpose based on its key returned no matches in cookiepedia.
    Out of {\respcookies} respawned cookies, 218 (11.58\%) were not classified by cookiepedia.
    %\NB{out of 1,883 or out of 432?}
    \NB{what's the relation with 432? Give a complete picture, otherwise the reader is lost.}
    \item Unknown: The cookie is present in cookiepedia, but the purpose of the cookie is unknown. 
    %\NB{but the cookie is present in cookiepedia?}
    1,149 (61.02\%) cookies were classified as unknown.
    \item Strictly necessary: These cookies are necessary for the functionality of the website.
    149 (7.91\%) cookies were classified as strictly necessary
    \item Targeting/Advertising: These cookies are used for advertising purposes.
    197 (10.46\%) cookies were classified as targeting/advertising.
    \item Performance: These cookies collect information about how visitors use a website.
    153 (8.12\%) cookies were classified as performance
    \item Functionality: These cookies are used to remember user choices.
    17 (0.90\%) cookies were classified as functionality.
\end{itemize}


\textit{Conclusion:} From the observed results, we can derive that...

\AL{very strange to end the section abruptly without any conclusion. It would be way better to discuss now the violation of the RGPD for the cookie purpose. Do not defer the discussion to another section, it feels disconnected.}

\paragraph{Duration of respawned cookies:}
The duration of a given cookie -- persistent or session-- can contribute to define whether a cookie is either exempted or subject to consent. 
%\AL{I don't understand this sentence.}
%\IF{rewritten}
A \textit{session cookie} is a cookie that is automatically deleted when the user closes her browser, while a \textit{persistent cookie} is a cookie that remains stored in the user’s terminal device until it reaches a defined expiration date (which can be minutes, days or several years)". Several Data Protection Authorities and the European Data Protection Board define their positioning regarding the lifespan of cookies, as shown in Table \ref{fig:life_posi}. We observe that there is no clear definition on the lifespan of cookies; however, the following principles need to be analysed according to the purpose at stake. These are: principle of "fairness", "purpose limitation", "data minimization", "storage limitation" (Article 5(1) GDPR).

\CS{Are we going to figure out how these principles apply?}

\AL{it is not a figure, but a table. I am not sure the term stakeholder is clear. I would use \textit{Data Protection Authorities}}

\CS{we are still discussing if we keep the table or not; if we do, we will define it better, with the due references and caption.}

\NB{Moreover, the audience probably doesn't know that 29WP and EDPB is the same thing.Please add citations to the relevant sources in the table (that for now inserted as a figure).}


\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{figures/Picture1.png}
    \caption{Positioning of the European Data Protection Board and Data Protection Authorities on the lifespan of cookies}
    \label{fig:life_posi}
\end{figure*}


\NB{Cristiana, I think we should use the "reasonable expectation of the user" and apply it over session cookies. If such cookies get respawned, they violate reasonable expectations and its intended function and therefore are likely non-compliant... Or at least very problematic!}

\CS{indeed! we started to say it already in section 3 page 10. now we have all these principles here to sketch :/}


%The legacy of a cookie is directly impacted by its lifetime.
%\NB{what is a "legacy of a cookie"?}
%The lifetime of a given cookie -- persistent or session-- can determine if a cookie is either exempted or subject to consent. 




%Session cookies used for customization and authentication are exempted of consent. When used in a persistent way, these cookies  would require consent of the user.
%\NB{I don't agree with the last conclusion. Authentication cookies don't require consent... Probably this is only true for customisation - to check with Cristiana.}
 

Out of {\respcookies} respawned cookies, 465 (24.69\%) are session cookies and 1,418 (75.31\%) are persistent cookies (Table \ref{tab:overview_resp}).
%\NB{Again, it would be super interesting to see who is setting session cookies and then respawns them!}
%\IF{Done}

The 465 respawned cookies instances (host, key, value) belong to 353 cookies (host,key).
\AL{you give raw numbers and do not draw any interesting conclusions. WE already discussed that several times. What is your hypothesis? "respawn session cookies are infringing the DPA policies on cookies duration". How do you support this hypothesis? "we observe session cookies that are respawn". Is it enough? No, you must then study the duration of the respawn session cookies. May be they are just respawn for a couple of minutes, for a couple of hours, for a couple of days, or for a couple of weeks. They do not mean the same. Also, you do not convincingly show that these cookies have the potential to track users (the fact that you take one example by hand such as the rubiconproject is not convincing enough). What is their entropy, which kind of information they store. Can you make a cloudtag of keys. May be it is just cookies setting the browser language, or some non critical information they just want to persist or a very low entropy session cookie.}

\begin{table}[!htbp]
    \centering
    \begin{tabular}{|p{3.5cm}|p{1cm}|p{1.7cm}|}
    \hline
\textbf{(Host, key)} & \textbf{Occu-rrence} & \textbf{Purpose}   \\ \hline
(rubiconproject.com, rsid)  &  515 & Unknown \\ \hline
(assets.rrz.unihamburg-.de, \_fionaapp\_session)  &  33 & Unknown  \\ \hline
(bh.contextweb.com ,  INGRESSCOOKIE) &  24  & Unknown\\ \hline
(bedbathandbeyond.com,  s\_sess)  &  9  & Performance \\ \hline
(key.com, s\_sess)  &  6 & Performance \\ \hline
(audible.fr, s\_sess)  &  6 & Performance \\ \hline
(www.dnb.no,    portal\_scriptable)  &  6 & Unknown  \\ \hline
(enterprise.com,    s\_sess)  &  5 & Performance  \\ \hline
(subway.com,    s\_sess)  &  4  & Performance \\ \hline
(snapdeal.com,    s\_sess)  &  3 & Performance  \\ \hline

    \end{tabular}
    \caption{Top 10 respawned session cookies.  \textit{Occurrence}: presents the number of websites where the cookie (host,key) was respawned. Purpose: cookiepedia corresponding purpose.}
    \label{tab:session}
\end{table}



Table \ref{tab:session} presents the top 10  respawned session cookies.
(Rubiconproject.com, rsid) cookies has been respawned in $515$ websites.
Rubiconproject states that: 

\say{\textit{rsid}: Session cookie that contains information about a device, including region (derived from IP address, not geolocation data), operating System, browser, etc., that is used during the ad inventory sale process} \cite{rubicon}.

In their policy, Rubiconproject defines the rsid cookie as a session cookie and do not state the fact that this cookie can be recreated.
\NB{This is big! A session cookie that gets respawned via fingerprinting used for ad inventory sale... We should have a complaint about this!
Imane, please share 5 top websites that have this practice from the 515 wbesites dataset!}

Among the top 10 respawned session cookies, 6 have as key s\_sess.
The s\_sess cookie is known as session web analytics cookies, provided and managed by Adobe Inc., and used to collect information about how visitors use websites. 
\NB{This is why it's important to see how many cookies share the same key! Why does s\_sess cookie belong to Adobe while you see it with differnet hosts?}

\begin{figure}[!ht]
    \centering
    \hspace*{-.9cm}                                  
    \includegraphics[width=0.7\textwidth]{figures/wordcloudsession.png}
    \caption{Word cloud of respawned session cookies keys.}
    \label{fig:wordcloud}
\end{figure}


\begin{table}[!htbp]
    \centering
    \begin{tabular}{|p{ 1.3cm}|c|p {2cm}|c|}
    \hline
    \textbf{Key} & \textbf{Service} & \textbf{Purpose} &  \\ \hline
         s\_ppn / s\_ppv / s\_ppvl & Adobe Analytics & Contains information about the current page and entry page to the website. & \cite{eib} \\ \hline

    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}





\subsubsection{Violation of GDPR}
\label{sec:violation}
Session cookies needed to provide a service explicitly requested by the user are initially exempted of consent. If respawned, these cookies could then be considered with a longer duration and henceforth would require consent of the user.

By using {\ourmethod}, a tracker can recreate session cookies after the expiration of the user session.
Hence, such cookies can be used for a longer duration than previously envisaged. This practice allows trackers to use the cookie for a persistent period of time without user's consent by exploiting the fact that the consent requirement is linked to the lifespan of cookies. Therefore, to evaluate the compliance of respawned cookies, we omit the duration of respawned cookie criteria and we focus on the purpose and the provenance.
\AL{I don't understand the logical link you make with the therefore. I don't understand why you do not consider anymore the cookie duration. I don't understand what is the use of table 7}



Even  if a website  owner  relies  on  self-claims  of “strictly  necessary” first-party  analytics,  the  29WP says that they are not strictly necessary to provide a functionality explicitly requested by the user, because the user can access all the functionalities provided by the website when such cookies are disabled. As a consequence, these cookies do not fall under the exemption of consent if they are used in a third party context.

Performance cookies are used to provide to the website owner statistics about their website. Theses cookies are providing analytics service hence, according to the 29WP are exempted from consent when used in a first party context \cite{}.\AL{so what?}

According  to  the 29WP, the short term functionality cookies used to keep track of users choices are exempted of consent. However, if used for a longer duration, these cookies will not be exempted of consent. The studied cookies are respawned, hence we consider that all cookies including session ones are persistent, therefore all functionality cookies are subject to consent. 
\AL{to make a strong claim, you must assess how long these cookies are respawn.}

In total, we found $301$ cookies violating GDPR.








\subsection{Entropy}



Different features contain different amount of information and hence contribute differently to uniqueness of each user.


\paragraph{\textbf{Entropy: }}
Entropy is used to evaluate how unique is a fingerprint.
The higher the entropy, the more unique is the fingerprint.

In this study we used the  shanon entropy calculated by Gómez-Boix et al \cite{gomezboix-www-2018}.
%The normlized entropy does not depend on the size of the studied dataset.
It is defined as follow:
  \[H(X) = -\sum p(X)\log p(X) \]
%\[ H[X]/ Hn \]

Where (Hn=$log_2$(M) ) and  M is the number of fingerprint in the dataset




\textbf{Assumption}: 
We assume that all features are independent.
Hence, we consider that:

\[ H[x,y] = H[X] + H[Y]  \] 



\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=.8\textwidth]{figures/top_used_entro_features.png}
    \caption{Top 20  features  with the highest entropy used in   fingerprinting based respawning in Alexa top {\websites}. In the x axis, we present (Features used, Entropy)}
    \label{fig:entropy}
\end{figure*}

In total, we have 4,294,967,296 possible IP address.
Which correspond to an entropy of 32.
For the geolocation, we assume that every person in the world has a different geolocation, 
and so we associate to the geolocation an entropy of 32.86
We have 167 features combinations used.



Figure \ref{fig:entropy} presents the top 20  features combinations with the highest entropy used in  {\ourmethod}.

All features combined have an entropy of 88.91. Which means that using all studied features one can uniquely identify ${2^{88.91}}$ users which is bigger than the world population (${2^{32.74}}$).



\subsection{Respawned cookies lifetime}

%Cookies are often categorized whether they are “session cookies” or “persistent cookie”~\cite{X}, "first party" or "third party". Accordingly, a “session cookie” is automatically deleted when the user closes his browser, while a “persistent cookie” remains stored in the user’s terminal device until itreaches a defined expiration date (which can be minutes, days or several years in the future).

We assume that short-termed cookies -- needed to provide a service explicitly requested by the user (and hence initially exempted of consent)--, if respawned, these could then be considered with a longer duration and henceforth would requiring consent of the user.\footnote{Regarding user interface customization cookies (also known as "preferences" or "personalization", the intention of the user could not be interpreted as a preference to
remember that choice for longer than a browser session (or no more than a few additional
hours). As such only session (or short term) cookies storing such information are exempted.} 
%As observed in section 3, the 29WP \cite{X} states that  specific purposes are needed to provide a service explicitly requested by the user, normally used along the duration of a session.
These can, for example, consist of users-input which are used to keep track of the user’s input (session-id) when
filling online forms over several pages, or as a
shopping cart, to keep track of the items the user has selected by clicking on a button.


By using {\ourmethod}, a controller can recreate session cookies after the expiration of the user session.
Hence, such cookies can be used for a longer duration than previously envisaged. 




We found that out of {\respcookies} respawned cookies, 465 (24.69\%) are session cookies.
The 465 respawned cookies instances (host,key,value) belong to 353 cookies (host,key).

\begin{table}[!htbp]
    \centering
    \begin{tabular}{|p{3.5cm}|p{2cm}|p{1.2cm}|}
    \hline
\textbf{Host} & \textbf{Key} & \textbf{Occu rrence}   \\ \hline
rubiconproject.com  &  rsid  &  515  \\ \hline
assets.rrz.uni-hamburg.de  &  \_fionaapp \_session  &  33  \\ \hline
bh.contextweb.com  &  INGRE-SSCOOKIE  &  24  \\ \hline
bedbathandbeyond.com  &  s\_sess  &  9  \\ \hline
key.com  &  s\_sess  &  6  \\ \hline
audible.fr  &  s\_sess  &  6  \\ \hline
www.dnb.no  &  portal \_scriptable  &  6  \\ \hline
enterprise.com  &  s\_sess  &  5  \\ \hline
subway.com  &  s\_sess  &  4  \\ \hline
snapdeal.com  &  s\_sess  &  3  \\ \hline

    \end{tabular}
    \caption{Top 10 respawned session cookies.  \textit{Occurrence}: presents the number of websites where the cookie (host,key) was respawned.}
    \label{tab:session}
\end{table}



%A session cookie get deleted when the user close her browser.
%Unlike session cookies where no expiration date is associated to the cookie, 
%persistent cookies have an expiration date and are get deleted within this last.
Table \ref{tab:session} presents the top 10  respawned session cookies.
Rubiconproject.com rsid cookies has been respawned in $515$ websites.
Rubiconproject states that: 

\say{\textit{rsid}: Session cookie that contains information about a device, including region (derived from IP address, not geolocation data), operating System, browser, etc., that is used during the ad inventory sale process} \cite{rubicon}.


We present the lifetime of the persistent respawned cookies in Figure \ref{fig:lifetime}.
\IF{Cristiana: what is considered as short termed cookies from a legal perspective}
\IF{To do: split tp and fp in figure 8}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/lifetime_features.png}
    \caption{Persistent respawned cookies lifetime \textit{Out of {\respcookies} respawned cookies, 1418 are persistent.} }
    \label{fig:lifetime}
\end{figure}

\IF{Done here}
\CS{explain if these respawned cookies are first or third party, as the need for 'consent exemption' varies}

\clearpage

\subsection{The respawning ecosystem}
A respawn cookie is either set as a \emph{First party} or a \emph{Third party} cookie.
\emph{First party} cookies are set in the users browser by the website explicitly 
visited by the user or programmatically by the third party script included in the website %(due to SOP). 
(due to the the Same Origin Policy (SOP) \cite{SameOriginPolicy}).
When used in isolation, 
first-party cookies %allow third parties % companies 
are capable to track users \emph{only within one website}.
%
\emph{Third party} cookies are set either (1) in the HTTP response by any third party content 
(images, html files or even at the delivery of scripts); or (2) programmatically via 
scripts operating from a third party iframe. 
Third party cookies allow third parties to %collect user's browsing history 
track users \emph{cross-websites}~\cite{Roes-etal-12-NSDI}.

% where gives an idea about the impact and the senstivity of the information collected. the who is linked to the use or the purpose of the behavior.
To study the interaction between the cookie owner (the tracker) and the website where the cookie is set, we excluded first party respawned cookies where the tracker and the website are identical and we focused on third party respawned cookies.

%\AL{why don't you call the host the tracker. The one who sets the cookie is the tracker, and the tracker can be a first party or a third party. The term host is confusing to me,}
%\IF{Done}


\begin{figure*}[!hbtp]
    \centering
    \hspace*{-.8cm}%
    %\includegraphics[width=1\textwidth]{figures/cat_relation_tp.png}
        \includegraphics[width=1\textwidth]{figures/map.png}
    \caption{ Categorization of respawned websites and respawned  cookies hosts in Alexa top 5,000 websites. \textit{ Top 50 third party relations. $-$: Links the category of the tracker to the category of the website where the cookie was set. We only consider third party relations where the tracker is different from the website. The arrow weight is proportional to the number of times the relation between the two categories occurs in our dataset. } }
    \label{fig:webCatcom}
\end{figure*}
\AL{what is the arrow scale (linear?) and the absolute value of the largest arrow (can we have the scale in legend). Also I would present Website on the left (name the column Websites so that you can remove the site\_ tag in each name, and on the right the trackers, name again the column Third party trackers}

The respawn website, is the website 
%that includes the respawned cookie and is directly 
that includes the trackers that sets the respawn cookie. The respawn website is directly visited by the user. 
%\AL{A web site does not include a cookie, it contains a third party tracker that sets the cookie?}
%\IF{DOne}

Hence, the category of the respawn website indicates the sensitivity of the information collected about the user on this given website. 
Whereas, the tracker, is the respawn cookies owner. Hence, the tracker's category potentially indicates the category of the party that collects the data, and even the purpose of the data collection.
To present who is respawning cookies in what category of websites, 
we categorized both the third party trackers and websites that include these cookies (see Figure \ref{fig:webCatcom}).   

From Figure \ref{fig:webCatcom} we see that, as expected, \textit{Business} is the most prominent host's category. 
The strongest relation is (\textit{Business}, \textit{General news}).
Most of the {Business} hosts are respawning cookies in news websites known for deploying third parties and ads more than other categories.
However, we also notice that the business hosts respawn cookies in other categories with different sensitivity degrees such as Job search  and profanity websites.

Business and Web Ads are most likely respawning third party cookies to guarantee a sticky tracking allowing them to collect information about the users  and recreate a more complete history of the user's browsing.
However, in addition to Business and Web Ads, we notice that hosts from other categories such as Internet Services are actively respawning cookies on different websites categories.

\AL{take home message}
%\AL{use a two column camera ready like template}

\subsection{Respawned cookie purposes}
In this section, we analyse the purposes of respawned cookies to understand whether they are subject of consent or not. 
As the 29WP (WP194) exposes, ‘it is the purpose and the specific implementation or processing being achieved that must be used to determine whether or not a cookie can be exempted from consent’.

We found a total of {\respcookies} respawned cookies and we have pursued our analysis in two ways: (1) considering the purposes of the top 5 respawned cookies (2) applying the Cookiepedia cookie purposes classification to the measurements we have performed;


%We analysed the purpose of respawned cookies to check if they require consent.

\subsubsection{Purposes of top 5 respwaned cookies}

We manually analyzed the purpose of the top 5 respawned cookies (Table \ref{tab:top5}).
We found that according to the declared cookie policy, 
2 out of the 5 cookies are used to store information about the device characterstics,
2 cookies are used to store anonymous data related to the user's visits to the website,
and the last cookie do not give a clear description of the purpose of the cookie.

\begin{table*}[!htb]
    \centering
    \begin{tabular}{|p {4cm}| p {9 cm}|}
    \hline
    \textbf{Cookie} & \textbf{Purpose} \\ \hline
     (rubiconproject.com ,rsid) & Session cookie that contains information about a device, including region (derived from IP address, not geolocation data), operating System, browser, etc., that is used during the ad inventory sale process \cite{rubicon}. \\ \hline
  (casalemedia.com,CMPS) &  Collects anonymous data related to the user's visits to the website, such as the number of visits, average time spent on the website and what pages have been loaded , with the purpose of displaying targeted ads \cite{casalmedia}. \\ \hline

(smartadserver.com,pbw)  & 	To target browsers, OS or screen size \cite{smartadserver}. \\ \hline

(casalemedia.com,CMDD) & Collects anonymous data related to the user's visits to the website, such as the number of visits, average time spent on the website and what pages have been loaded , with the purpose of displaying targeted ads \cite{casalmedia}. \\ \hline

(pubmatic.com, pi) &  This cookie enables us to determine which set of pixels needs to be executed on the browser \cite{pubmaticpolicy}. \\ \hline
    \end{tabular}
    \caption{Purposes of the  top 5 respawned cookies.}
    \label{tab:top5}
\end{table*}


\subsubsection{Cookiepedia cookie purposes classification}
To extract the purpose of {\respcookies} respawned cookies, we  automatized the cookiepedia service \cite{cookiepedia}.
We made an automatic search of the cookie purpose based on cookies keys.
The {\respcookies} respawned cookies use a set of $432$ unique keys.
For every key, we sent an automatic request to cookiepedia, then we extracted the corresponding purpose.
\iffalse
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.5\textwidth]{figures/cookies_purposes.png}
    \caption{Purposes of the respawned cookies keys based on cookiepedia cookies classification. \textit{5.56\% of the respawned cookies are used for targeting and advertising purposes that requires user's consent.}}
    \label{fig:purposes}
\end{figure}
\fi

\begin{figure}[!htbp]
\centering
\subfloat[%Comparing to 
{First-party respawned cookies}\label{fig:compareELEP}]{\includegraphics[width=0.35\textwidth]{figures/cookies_purposes_fp.png}}

\subfloat[%Comparing to 
Third party respawned cookies\label{fig:compareDISC}]{\includegraphics[width=0.35\textwidth]{figures/cookies_purposes_tp.png}}
\caption{ {\normalfont}
Purposes of the respawned cookies  based on cookiepedia cookies classification. \textit{6.60\% of the first party and 17.07\% of the third party respawned cookies  are used for targeting and advertising purposes that requires user's consent.}} %({\totaldomainssucc} domains).}
\label{fig:purposes} 
\end{figure} 

We illustrate our results in Figure \ref{fig:purposes}, thereby depicting the purposes of  respawned cookies.
Out of {\respcookies} respawned cookies, $1,665$  were classified by cookiepedia.
Among which, 832 are classified as third-party cookies and 833 as first-party cookies.
We consider that a respawned cookie is a third party cookie, if it is used in  third party context in at least one of the respawned websites.
We found that the purpose of 66.27\% of first-party  and 71.75\% of third-party respawned cookies is unknown, 9.24\% and 8.65\% are respectively strictly necessary, hence exempted from the user's consent, and 6.60\%  and 17.07 of respawned cookies are used for targeting and advertising.
%The cookies keys used for targeting and advertising correspond to $197$(10.46\%) cookies. 
These targeting and advertising cookies are violating the lawfulness principle of the GDPR since no consent was given in our study.
....



\CS{we need also to explain what cookiepedia means with "functionality", performance", "strict necessary" purposes, maybe using a table}




\iffalse
We present this list of $11$ unique (host,key) in Table \ref{tab:all_features}.


%\AL{poor wording}
\begin{table}[!h]
    \centering
    \begin{tabular}{|p{3cm}|p{3.5cm}|}
    \hline
\textbf{Host} & \textbf{Key} \\ \hline    
citationmachine.net & ad\_config\_version \\ \hline
citationmachine.net &  al\_ff  \\ \hline
openclassrooms.com &  AWSELB  \\ \hline
openclassrooms.com & AWSELBCORS  \\ \hline
casalemedia.com & CMPRO  \\ \hline
bh.contextweb.com & INGRESSCOOKIE  \\ \hline
quantserve.com & d   \\ \hline
rubiconproject.com & vis15   \\ \hline
gsuite.google.com & APPS\_MARKETING \_SIGNALS  \\ \hline
www.kaspersky.ru & webserver\_id  \\ \hline
betweendigital.com & dc  \\ \hline

    \end{tabular}
    \caption{Respawned cookies using all features combined.}
    \label{tab:all_features}
\end{table}



Figure \ref{fig:feature500}  presents the set of features used with the top
500 cookies. The ranking is based on the number of features used with the cookie.
\fi





